A Separation Result Between Data-oblivious and Data-aware Poisoning Attacks

Poisoning attacks have emerged as a significant security threat to machine learning algorithms. It has been demonstrated that adversaries who make small changes to the training set, such as adding specially crafted data points, can hurt the performance of the output model. Some of the stronger poisoning attacks require the full knowledge of the training data. This leaves open the possibility of achieving the same attack results using poisoning attacks that do not have the full knowledge of the clean training set. In this work, we initiate a theoretical study of the problem above. Specifically, for the case of feature selection with LASSO, we show that full-information adversaries (that craft poisoning examples based on the rest of the training data) are provably stronger than the optimal attacker that is oblivious to the training set yet has access to the distribution of the data. Our separation result shows that the two setting of data-aware and data-oblivious are fundamentally different and we cannot hope to always achieve the same attack or defense results in these scenarios.

==> Conc.tex <==
\section{Conclusion} \label{sec:conc}

In this paper we initiated a formal study of the power of oblivious adversaries who do not have any information about the training set in comparison with full-information adversaries who know the training data completely before adding poison points to it. 

Our main result proved a separation between the two threat models  by constructing a sparse linear regression problem for which Lasso estimator is robust against oblivious adversaries that aim to add a non-relevant features to the model with certain poisoning budget. On the other hand, for the same problem, we prove that full-information adversaries, with the same budget,  can find specific poisoning examples based on the rest of the training data in such a way that they can successfully add non-relevant features to the model.
Our work sheds light on an important and yet subtle aspect of modeling the threat posed by poisoning adversaries. 

Another contribution of our work was to study poisoning attacks in the context of model recovery and for a sparse linear regression problem, where the goal of the adversary is something different from increasing the population risk (or failure probability on a particular example).

For future work, a general direction is to explicitly study other subtle aspects of poisoning attacks that are implicit in previous work. A specific direction is to study the power of oblivious poisoning attacks when the goal of the adversary is to increase the population risk or the probability of a bad event (i.e., targeted poisoning) as these are the most common goals of poisoning attacks studied in the literature. Specifically, consider a bad property $B$ over the hypothesis class $\cH$, and a learning algorithm $L\colon Z^n \to \cH$. Does there exist a distribution $D$ over $Z^n$ and a poisoning size $p$ such that 
\begin{align*}
    \max_{A\in \set{f \colon \cH \to Z^p}} \Pr_{\substack{T\gets D;\\ h\gets L(T);\\ T'\gets A(h)}}\left [B\left(L\left(\concatv{T}{T'}\right)\right)=1\right]
\end{align*}
is much smaller than  
\begin{align*}
    \max_{A\in \set{f \colon Z^n \to Z^p}} \Pr_{\substack{T\gets D;\\ T'\gets A(T)}}\left [B\left(L\left(\concatv{T}{T'}\right)\right)=1\right].
\end{align*}
Finally, as discussed in the introduction, our results show that \emph{online} adversaries who only know the training data till a particular point in time, fall somewhere between full information and oblivious attacks. Can we formalize such attacks for model recovery and prove that they are more/less powerful than either of full information or oblivious settings?

==> experiments_details.tex <==
\section{More Details about Feature Selection Experiments}\label{sec:exp_details}
In this section, we give further details about the particular construction for our model recover experiments in Section \ref{sec:experiments} and the real-world experiments for larger datasets. 

% \subsection{Synthetic Experiments: Constructed Dataset}\label{sec:synthetic_details}
% We construct our dataset exactly as in Construction \ref{const:1}, so we have:

% $$\concat{X}{Y}=\concatt{X_0}{Y_0}{X_1}{Y_1} \in  \R^{(n+\lambda - k)\times d},$$ 

% In particular, we set $n = 1000,$ $d = 10^5$, $k = 1$, and $s = 5$ in our construction, so our dataset has $999 + \lambda$ rows and $10^5$ features. We set $\sigma = 1/4$ for our noise vector $W,$ which determines $\lambda.$ We use scikit-learn's implementation of Lasso \cite{scikit-learn}, setting the regularization parameter to $2\lambda / n$, as defined in Section \ref{sec:intro}. Due to numerical instability, we use $\lambda = 121$ (which is slightly higher than the $4\sigma \sqrt{n \log(d)}$ in the construction) to instantiate the dataset, giving us:

% $$\concat{X}{Y}=\concatt{X_0}{Y_0}{X_1}{Y_1} \in  \R^{(n+\lambda - k)\times d} \in \R^{1,120 \times 100, 000}$$

% where $X_0, Y_0, X_1,$ and $Y_1$ are given in Construction \ref{const:1}.

\subsection{Synthetic Experiments: Natural Gaussian Dataset}\label{sec:synthetic2_details}
We construct the natural Gaussian dataset by sampling from $\mathcal{N}(0, 1)^{n \times d},$ which gives us:

\begin{align*}
    X = \left[ \begin{array}{ccc}
   \mathcal{N}(0, 1) & \dots & \mathcal{N}(0, 1) \\
   \vdots & \ddots & \vdots  \\
   \mathcal{N}(0, 1) & \dots
   & \mathcal{N}(0,1) \\
  \end{array} \right] \in \mathbb{R}^{n \times d}
\end{align*}

We let $n = 300$ and $d = 5 \times 10^5$ and sample our noise vector $W$ from $\mathcal{N}(0, \sigma^2)^{n \times 1}$ with $\sigma = 1/2$. Let $\theta^* \in [0,1]^{d}$ be the optimal parameter vector with the first $s = 5$ coordinates with non-zero values and the last $d - s$ coordinates equal to 0. With these parameters, we set the target variables to be $Y = X\theta^* + W$. For the Lasso estimator itself, we use $\lambda = 4\sigma\sqrt{n \log(d)}$ as in Theorem \ref{thm:LassoRobustRecovery}.

\subsection{Experiment with Real-world Data}\label{sec:realworld_details}
For our real-world datasets, we use four datasets typically used in the model recovery setting:

\begin{itemize}

    \item \textbf{Boston.} \cite{boston} (506 examples, 13 features) The task in this dataset is to predict the median value of a house in the Boston, Mass. area, given attributes that describe its location, features, and surrounding area. The outcome variable is continuous in the range $[0, 50].$
    \item \textbf{TOX.} \cite{tox} (171 examples, 5,748 features) The task in this dataset is to predict whether a patient is a myocarditis and dilated cardiomyopathy (DCM) infected male, a DCM infected female, an uninfected male, or an uninfected female. Each feature is a gene, and each example is a patient. The outcome variable is discrete in $\{1, 2, 3, 4\},$ for each of the four possibilities.
    \item \textbf{Prostate\_GE.} \cite{prostate} (102 examples, 5,966 features) The task in this dataset is to predict whether a patient has prostate cancer. Each feature is a gene, and each example is a patient. The outcome variable is binary in $\{0, 1\},$ for cancer or no cancer.
    \item \textbf{SMK.} \cite{tox} (187 examples, 19,993 features) The task in this dataset is to predict whether a smoker has lung cancer or not. Each example is a smoker, and each faeture is a gene. The outcome variable is binary in $\{0, 1\}$ for cancer or no cancer.
    \item \textbf{MNIST} We use MNIST data for feature selection. Each pixel number constitutes a feature and we want to recover a subsst of them that are more relevant.
\end{itemize}

In Figure, we show the effect of knowledge of the data on Boston and Prostate datasets. We did not report these two experiments in the main body.

\begin{figure}[ht]
\center
    %\includegraphics[scale=0.1]{Experiment/New_Experiments/boston.png}
    \includegraphics[scale=0.1]{Experiment/New_Experiments/boston.png}

    \includegraphics[scale=0.1]{Experiment/New_Experiments/PROSTATE.png}

     \caption{\textit{SMK and TOX Experiments.}}
     \label{fig:realworld_exp}
\end{figure}
% For the larger datasets, we see the same phenomenon as the Boston dataset in Section \ref{sec:experiments}, where there certainly exist unstable features that require a small number of rows to poison, and stable features that require a large number of rows, as shown in Figure \ref{fig:fulldataset_exp}. Even in subsets of 50 features from the full dataset, we see the same phenomenon, seen in \ref{fig:50dataset_exp}. For instance, in TOX, feature 106 requires less than 5 poison rows to add it to the dataset, while the average is 22 and the maximum number of rows is above 60. An non-oblivious adversary could exploit feature 106, while an oblivious adversary would pick a feature that takes 22 poison rows, in expectation. In Figure 3, we show the same phenomenon on each dataset for a subset of 50 features for visual clarity. 

%  \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{Experiment/final_fulldataset_appendix.png}
%      \caption{\textit{TOX, Prostate\_GE, SMK (full dataset).} We attacked all the features not in $\Supp(\hat{\theta})$, and plotted the number of rows needed to add feature $i$ to the dataset. The red horizontal line is the mean number of rows. The top figure shows Prostate\_GE, the middle TOX, and the bottom SMK.} 
%      \label{fig:fulldataset_exp}
% \end{figure}

%  \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{Experiment/50_fulldataset_appendix.png}
%      \caption{\textit{TOX, Prostate\_GE, SMK (50 features).} We choose a random subset of 50 features not in $\Supp(\hat{\theta})$, and plotted the number of rows needed to add feature $i$ to the dataset. The red horizontal line is the mean number of rows. The top figure shows Prostate\_GE, the middle TOX, and the bottom SMK. The red colored bar shows the $k$-unstable feature in the dataset that a non-oblivious adversary could exploit.} 
%      \label{fig:50dataset_exp}
% \end{figure}




==> experiments_details_FS.tex <==
\section{More Details about Feature Selection Experiments}\label{sec:exp_details_fs}

\paragraph{Attacking a specific feature:} For our experiments on feature selection we use the following attack similar to the attack described in Section \ref{sec:optimal-attack}. 
To attack a feature $i$ with $k$ examples, we use a dataset $\cS'=\concat{X'}{Y
 '}$ as follows:
\begin{align*}
    X' = \left[
    \begin{array}{cccc}
         0 & \dots & 1 & 0\\
         \vdots&\ddots &\vdots &\vdots\\
         0 & \dots & 1 & 0
    \end{array}
    \right] \in \mathbb{R}^{k \times d} 
    , 
    Y' = \left[
    \begin{array}{c}
          1\\
         \vdots\\
         1
    \end{array}
    \right] \in \mathbb{R}^{k \times 1}.
\end{align*}
The attack then adds $S'$ to the training set. Note that this attack is oblivious as it does not use the knowledge of the clean training set.

\paragraph{How to select the feature to attack?}
In total, the attack aims to find the feature that requires the minimum number of rows to add to $\Supp(\hat{\theta}),$ where $\hat{\theta}$ is the learned parameter vector from Lasso. From Section \ref{sec:optimal-attack} we know that the attack above is almost optimal for adding a specific feature. However, the attack still has to decide which feature to attack as some features are much more unstable than others. A question that might arise here is why  the power of data-oblivious and data-aware adversaries would change if the same underlying attack is used by both of them. The key here is that the data-aware adversary can search for the most vulnerable feature and target that feature specifically. However, the data-oblivious adversary has to choose the features that will \emph{probably} be unstable. Namely, the attack should sample multiple dataset from the distribution and identify which features get unstable more frequently. However, there could be a lot of entropy in the instability of different features which makes the job of oblivious adversary hard. 

Using this logic, we can even run experiment on partially-aware adversaries by only allowing them to see a random fraction of the training set. In this setting the adversary first tries to identify the unstable features by leveraging the part of the training set that it has access to. Specifically, the adversary first completes the dataset by randomly sampling from the distribution and combining it with the fraction of the data that it has access to. Then, it checks all the coordinates of this constructed dataset and identifies the one that requires the lowest number of attack samples, based on the attack described above. As the fraction of the known data increases, the approximation of stability of features decreases and the attacker can identify the unstable features with higher probability. This is the key in the decrease in the success of the attack when less data is known to the attacker. 


\paragraph{Datasets:} Here we give further details about the particular construction for our model recovery experiments in Section \ref{sec:experiments} and the real-world experiments for larger datasets. 

% \subsection{Synthetic Experiments: Constructed Dataset}\label{sec:synthetic_details}
% We construct our dataset exactly as in Construction \ref{const:1}, so we have:

% $$\concat{X}{Y}=\concatt{X_0}{Y_0}{X_1}{Y_1} \in  \R^{(n+\lambda - k)\times d},$$ 

% In particular, we set $n = 1000,$ $d = 10^5$, $k = 1$, and $s = 5$ in our construction, so our dataset has $999 + \lambda$ rows and $10^5$ features. We set $\sigma = 1/4$ for our noise vector $W,$ which determines $\lambda.$ We use scikit-learn's implementation of Lasso \cite{scikit-learn}, setting the regularization parameter to $2\lambda / n$, as defined in Section \ref{sec:intro}. Due to numerical instability, we use $\lambda = 121$ (which is slightly higher than the $4\sigma \sqrt{n \log(d)}$ in the construction) to instantiate the dataset, giving us:

% $$\concat{X}{Y}=\concatt{X_0}{Y_0}{X_1}{Y_1} \in  \R^{(n+\lambda - k)\times d} \in \R^{1,120 \times 100, 000}$$

% where $X_0, Y_0, X_1,$ and $Y_1$ are given in Construction \ref{const:1}.

\subsection{Synthetic Experiments: Natural Gaussian Dataset}\label{sec:synthetic2_details}
We construct the natural Gaussian dataset by sampling from $\mathcal{N}(0, 1)^{n \times d},$ which gives us:

\begin{align*}
    X = \left[ \begin{array}{ccc}
   \mathcal{N}(0, 1) & \dots & \mathcal{N}(0, 1) \\
   \vdots & \ddots & \vdots  \\
   \mathcal{N}(0, 1) & \dots
   & \mathcal{N}(0,1) \\
  \end{array} \right] \in \mathbb{R}^{n \times d}
\end{align*}

We let $n = 300$ and $d = 5 \times 10^5$ and sample our noise vector $W$ from $\mathcal{N}(0, \sigma^2)^{n \times 1}$ with $\sigma = 1/2$. Let $\theta^* \in [0,1]^{d}$ be the optimal parameter vector with the first $s = 5$ coordinates with non-zero values and the last $d - s$ coordinates equal to 0. With these parameters, we set the target variables to be $Y = X\theta^* + W$. For the Lasso estimator itself, we use $\lambda = 4\sigma\sqrt{n \log(d)}$ as in Theorem \ref{thm:LassoRobustRecovery}.

\subsection{Experiment with Real-world Data}\label{sec:realworld_details}


 For our real-world datasets, we use four datasets typically used in the model recovery setting.
\begin{itemize}

    \item \textbf{Boston.} \cite{boston} (506 examples, 13 features) The task in this dataset is to predict the median value of a house in the Boston, Mass. area, given attributes that describe its location, features, and surrounding area. The outcome variable is continuous in the range $[0, 50].$
    \item \textbf{TOX.} \cite{tox} (171 examples, 5,748 features) The task in this dataset is to predict whether a patient is a myocarditis and dilated cardiomyopathy (DCM) infected male, a DCM infected female, an uninfected male, or an uninfected female. Each feature is a gene, and each example is a patient. The outcome variable is discrete in $\{1, 2, 3, 4\},$ for each of the four possibilities.
    \item \textbf{Prostate\_GE.} \cite{prostate} (102 examples, 5,966 features) The task in this dataset is to predict whether a patient has prostate cancer. Each feature is a gene, and each example is a patient. The outcome variable is binary in $\{0, 1\},$ for cancer or no cancer.
    \item \textbf{SMK.} \cite{tox} (187 examples, 19,993 features) The task in this dataset is to predict whether a smoker has lung cancer or not. Each example is a smoker, and each faeture is a gene. The outcome variable is binary in $\{0, 1\}$ for cancer or no cancer.
    \item \textbf{MNIST} We use MNIST data for feature selection. Each pixel number constitutes a feature and we want to recover a subsst of them that are more relevant.
\end{itemize}

In Figure, we show the effect of knowledge of the data on Boston and Prostate datasets. We did not report these two experiments in the main body.

\begin{figure}[ht]
\center
    %\includegraphics[scale=0.1]{Experiment/New_Experiments/boston.png}
\begin{subfigure}[b]{0.48\linewidth}
    \includegraphics[scale=0.1]{Experiment/New_Experiments/boston.png}
\end{subfigure}
\begin{subfigure}[b]{0.48\linewidth}
    \includegraphics[scale=0.1]{Experiment/New_Experiments/PROSTATE.png}
\end{subfigure}
     \caption{\textit{SMK and TOX Experiments.}}
     \label{fig:realworld_exp_app}
\end{figure}
% For the larger datasets, we see the same phenomenon as the Boston dataset in Section \ref{sec:experiments}, where there certainly exist unstable features that require a small number of rows to poison, and stable features that require a large number of rows, as shown in Figure \ref{fig:fulldataset_exp}. Even in subsets of 50 features from the full dataset, we see the same phenomenon, seen in \ref{fig:50dataset_exp}. For instance, in TOX, feature 106 requires less than 5 poison rows to add it to the dataset, while the average is 22 and the maximum number of rows is above 60. An non-oblivious adversary could exploit feature 106, while an oblivious adversary would pick a feature that takes 22 poison rows, in expectation. In Figure 3, we show the same phenomenon on each dataset for a subset of 50 features for visual clarity. 

%  \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{Experiment/final_fulldataset_appendix.png}
%      \caption{\textit{TOX, Prostate\_GE, SMK (full dataset).} We attacked all the features not in $\Supp(\hat{\theta})$, and plotted the number of rows needed to add feature $i$ to the dataset. The red horizontal line is the mean number of rows. The top figure shows Prostate\_GE, the middle TOX, and the bottom SMK.} 
%      \label{fig:fulldataset_exp}
% \end{figure}

%  \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{Experiment/50_fulldataset_appendix.png}
%      \caption{\textit{TOX, Prostate\_GE, SMK (50 features).} We choose a random subset of 50 features not in $\Supp(\hat{\theta})$, and plotted the number of rows needed to add feature $i$ to the dataset. The red horizontal line is the mean number of rows. The top figure shows Prostate\_GE, the middle TOX, and the bottom SMK. The red colored bar shows the $k$-unstable feature in the dataset that a non-oblivious adversary could exploit.} 
%      \label{fig:50dataset_exp}
% \end{figure}


==> extra.tex <==
\section{Setting and Questions} \label{sec:prelim}


Story and the steps.
\begin{itemize}
    \item In sparse learning, we want to recover a sparse solution to a (noisy) system of equations. More generally, in model recovery, we want to find a specific function that we know it exists, existentially.
    \item In a poisoning attack tailored for this setting, we want to make the learner go as far as possible from the actual model that shall be recovered. In the case of sparse learning, this "distance" could be modeled using Hamming distance. \MohNote{Is this type of poisoning defined at all?}
    \item In the formulation above, instability, and poisoning against model recovery, are very much related and probably we can formalize the connection fully.
    \item Then, we will have a way to define poly-time vs. info theoretic attacks on instability as well as poisoning for model recovery.
    \item Finally, we want to separate the two (poly time vs. info theoretic) using specific examples/candidates by perhaps reducing them to hard problems in lattices/decoding random linear codes.
\end{itemize}

\noindent Related papers:
\begin{itemize}
    \item \url{http://proceedings.mlr.press/v30/Guha13.pdf}
    \item \url{http://users.ece.utexas.edu/~cmcaram/pubs/XuMannorCaramanis.NFLAllerton.pdf}
    \item Wainwright \url{https://arxiv.org/abs/0910.2042}
    \item Nisheet Vishnoi \url{https://arxiv.org/abs/1902.07823}
    
    \item Book by Wainright-Tshibrani
    \url{https://web.stanford.edu/~hastie/StatLearnSparsity_files/SLS_corrected_1.4.16.pdf}
    
    \item Medical application of sparse estimation
    \url{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC3783968/}
    
\end{itemize}


\section{The attack of UT Austin paper}
\begin{definition}
 A linear regression algorithm $A$ is sparse if for any given set of labeled examples $[X , Y]$   such that the $i$th and $j$th column of $X$ are exactly the same, its  output model is zero on either $i$th or $j$th coordinate. This means that the algorithm is able to eliminate the redundant columns. Note that $\ell_k$ regularizers for any $k\geq1$ do not impose this condition.
\end{definition}

The attack is trying to show that a sparse regressor cannot be stable. The idea is very simple. Asumme we have a stable algorithm $A$, consider a set of labeled examples $[X,Y]$ where $X\in R^{n\times p}$. Now consider another set of examples $[X',Y]$ where $X' = (X|X) \in \R^{n\times 2p}$. Assume the output of $A$ on $[X',Y]$ is $\theta'\in \R^{2p}$ and is 0 on all the first $p$ coordinates. Let $\theta$ be the second $p$ coordinates of $\theta'$, namely $\theta' = (0^p | \theta)$. And consider an example $(z,0)\in \R^{p+1}$ such that $\theta$ performs bad on $(z,0)$. Now if we add the point $z'=[(0^p,z), 0]$ to our set of examples $[X', Y]$ and train $A$ on that, we get the model $\theta'' = (\theta|0^p)$ which has Loss $0$ on the added point $z'$ and performs the same as $\theta'$ on all other examples in $X'$. This means that the loss of the output of $A$ on $z'$ changes significantly when adding $z'$ to the training set which means $A$ is not stable.      
